Proof-Carrying Parameters in Certified Symbolic Execution: The Case Study of Antiunification

Symbolic execution uses various algorithms (matching, (anti)unification), whose executions are parameters for proof object generation. This paper proposes a generic method for generating proof objects for such parameters. We present in detail how our method works for the case of antiunification. The approach is accompanied by an implementation prototype, including a proof object generator and a proof object checker. In order to investigate the size of the proof objects, we generate and check proof objects for inputs inspired from the K definitions of C and Java.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Vlad Rusu (Ed.) Sixth Working Formal Methods Symposium (FROM 2022)\\
EPTCS 369, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.369.1}{10.4204/EPTCS.369.1}}
\pdfoutput=1

